HyperGuider: Virtual Reality Framework for Interactive Path Planning of Quadruped Robot in Cluttered and Multi-Terrain Environments

Quadruped platforms have become an active topic of research due to their high mobility and traversability in rough terrain. However, it is highly challenging to determine whether the clattered environment could be passed by the robot and how exactly its path should be calculated. Moreover, the calculated path may pass through areas with dynamic objects or environments that are dangerous for the robot or people around. Therefore, we propose a novel conceptual approach of teaching quadruped robots navigation through user-guided path planning in virtual reality (VR). Our system contains both global and local path planners, allowing robot to generate path through iterations of learning. The VR interface allows user to interact with environment and to assist quadruped robot in challenging scenarios. The results of comparison experiments show that cooperation between human and path planning algorithms can increase the computational speed of the algorithm by 35.58% in average, and non-critically increasing of the path length (average of 6.66%) in test scenario. Additionally, users described VR interface as not requiring physical demand (2.3 out of 10) and highly evaluated their performance (7.1 out of 10). The ability to find a less optimal but safer path remains in demand for the task of navigating in a cluttered and unstructured environment.

==> reviews.tex <==


% In addition, the results of the experiment showed that users were divided into two groups according to the final path (Fig.~\ref{fig:exp3_paths}). For example, seven users provided paths that are closely resembles the path computed without interaction, while others decided to navigate the robot by longer paths. %Such kind of behavior can be useful in scenarios of navigation in cluttered and unstructured environments where the shortest path go through unstable structures or areas with potential danger for a quadruped robot.

% \begin{figure}[htbp]
% \begin{center}
% \centerline{\includegraphics[width=0.5\textwidth]{figures/exp3_pathTypes.png}}
% \caption{Examples of final paths generated autonomously (green line) and with user assistance (red and blue lines).}
% \label{fig:exp3_paths}
% \end{center}
% \end{figure}
